Approximate Equilibrium Computation for Discrete-Time Linear-Quadratic Mean-Field Games

While the topic of mean-field games (MFGs) has a relatively long history, heretofore there has been limited work concerning algorithms for the computation of equilibrium control policies. In this paper, we develop a computable policy iteration algorithm for approximating the mean-field equilibrium in linear-quadratic MFGs with discounted cost. Given the mean-field, each agent faces a linear-quadratic tracking problem, the solution of which involves a dynamical system evolving in retrograde time. This makes the development of forward-in-time algorithm updates challenging. By identifying a structural property of the mean-field update operator, namely that it preserves sequences of a particular form, we develop a forward-in-time equilibrium computation algorithm. Bounds that quantify the accuracy of the computed mean-field equilibrium as a function of the algorithm's stopping condition are provided. The optimality of the computed equilibrium is validated numerically. In contrast to the most recent/concurrent results, our algorithm appears to be the first to study infinite-horizon MFGs with non-stationary mean-field equilibria, though with focus on the linear quadratic setting.

==> Section5.tex <==

In this section a model-free two timescale Q-learning based algorithm is proposed to iteratively recover the equilibrium control. The two timescale algorithm involves updates at faster and slower timescales. The faster timescale involves Q-learning for a \textit{quasi-fixed} mean-field and the slower timescale is regarding update of the mean-field. Notice that as in standard two timescale formulation, the mean-field is not actually fixed but \textit{appears} to be fixed, to the faster timescale.
\aznote{This is how this section should be structured. First show that the two timescale algorithm follows the linear part of the $\tau$-latent LTI mean-fields. Then show how following the $\tau$-latent LTI mean-fields is synonymous with following the equilibrium mean-field but for time $\geq t$.}

Section \ref{subsec:QlearningLQR} solves the problem of tracking $\tau$-latent mean-fields for $t \geq \tau$, in a model-free setting. This is achieved through casting the problem into a Q-learning problem. Then some useful properties of the update of the Q-function are obtained. Section \ref{subsec:TTSRL} details how this Q-learning is used in a two timescale algorithm to approach the equilibrium control for the generic agent. This involves an unbiased estimate of the operator $\mathcal{T}^L$.

\subsection{Q-learning for stochastic LQR} \label{subsec:QlearningLQR}

Just as finding the cost-minimizing control for a $\tau$-latent LTI mean-field for $t \geq \tau$ can be cast as a stochastic LQR problem (Section \ref{sec:PI}); the model-free version of this problem, %(learning the cost-minimizing control for a $\tau$-latent LTI mean-field and $t > \tau$) 
can be cast as Q-learning for stochastic LQR. Towards this end this section obtains some useful properties of the Q-function and details the update of the Q-function, in a stochastic LQR setting. First the form of the Q-function and its optimal control is obtained in the following lemma. Its proof is provided in the appendix.
\begin{lemma} \label{lem:Q_func_LQR}
	The $Q$-function of an infinite horizon stochastic LQR problem \eqref{eq:augdynamics}-\eqref{eq:augcostfunc} has the form,
	\begin{equation}
	Q(X_t, u_t) = \left[ \begin{array}{c} X_t \\ u_t \end{array} \right]^T H \left[ \begin{array}{c} X_t \\ u_t \end{array} \right] + r
	\end{equation}
	Moreover, the control which minimizes $Q(X_t, u_t)$ has the form $u_t = L^* X_t$ where,
	\begin{equation} \label{eq:L_t}
	L^* = - \left( H^{uu} \right)^{-1} H^{ux} \text{ where } H = \left[ \begin{array}{cc} H^{xx} & H^{xu} \\ H^{ux} & H^{uu} \end{array} \right]
	\end{equation}
\end{lemma}



%\subsection{Q-learning for stochastic stochastic LQR}

Now consider $Q^{k}$ as an approximation of the function $Q$. As $k \rightarrow \infty$, $Q^{k}$ is expected to converge to $Q$. $Q^{k}$ is defined to have a form similar to $Q$,
\begin{equation} \label{eq:Q_func}
Q^{k}(X_t, u_t) = \left[ \begin{array}{c} X_t \\ u_t \end{array} \right]^T H^{k} \left[ \begin{array}{c} X_t \\ u_t \end{array} \right] + r^{k}
\end{equation}
where $H^{k}$ approximates $H$ and $r^{k}$ approximates $r$. The update of the $Q^k$ is given by,
\begin{multline} \label{eq:Qupdate}
Q^{k+1}(X_t, u_t) = \left[ \begin{array}{c} X_t \\ u_t \end{array} \right]^T \left[ \begin{array}{cc} S & 0 \\ 0 & c_2 \end{array} \right] \left[ \begin{array}{c} X_t \\ u_t \end{array} \right] + \\
\gamma \min_{u_{t+1}} Q^{k}(X_{t+1}, u_{t+1})
\end{multline}
This update involves update of $H^k$ and $r^k$ %The update rules for $H^k$ and $r^k$ are presented in the lemma below,
%\begin{lemma} \label{lem:Hk_rk_update}
%If $Q^k$ is defined as in equation \eqref{eq:Q_func}, then the update rules for $H^k$ and $r^k$ are,
%\begin{align}
%& H^{k+1} =  \left[ \begin{array}{cc} S & 0 \\ 0 & c_2 \end{array} \right] + \gamma Y^{k} = \left[ \begin{array}{cc} S & 0 \\ 0 & c_2 \end{array} \right] + \\
%& \gamma  \left[ A \hspace{0.2cm} B \right]^T
%\left[ \begin{array}{c} I \\ L^{k} \end{array} \right]^T H^{k} \left[ \begin{array}{c} I \\ L^{k} \end{array} \right]  \left[ A \hspace{0.2cm} B \right] \nonumber
%\end{align}
%and
%\begin{multline}
%r^{k+1} = \gamma \left( 2 \left( A X_t + B u_t \right)^T P^{k} \bar{\sigma} \omega_t \right. \\ \left. + (\bar{\sigma} \omega_t)^T P^{k} \bar{\sigma} \omega_t + r^{k} \right)
%\end{multline}
%\end{lemma}
and under this rule $H^k \xrightarrow{k \rightarrow \infty} H$ as shown in the following lemma.
\begin{lemma} \label{lem:H^k->H}
	Given the update of $Q^k$ as in equation \eqref{eq:Qupdate}, $H^k \rightarrow H$ as $k \rightarrow \infty$. Moreover if we define an operator $\mathcal{H}$, such that $H^{k+1} = \mathcal{H} (H^k)$ then, $\mathcal{H}$ is contractive.
\end{lemma}
Proof can be found in appendix. The update of $r^k$ on the other hand  is a stochastic update and so convergence of $r^k$ cannot be proved. Nonetheless, some other properties of the update of $r^k$ are explored in the following lemma. These properties help in obtaining convergence results in the two timescale algorithm.
\begin{lemma} \label{lem:r^k->r}
	Let us define a deterministic version of the stochastic update of $r^k$,
	\begin{equation} \label{eq:r^k_update_determ}
	\mathbf{r}^{k+1} = \EE \left[ r^{k+1} \mid \mathbf{r}^{k} \right] %= \gamma \tr(\bar{\sigma}^T P_n \bar{\sigma}) + \gamma \mathbf{r}^k
	\end{equation}
	Then $\mathbf{r}^k \rightarrow r$ as $n \rightarrow \infty$. Moreover,
	$
	\EE \left[ r^{k+1} - \EE \left[ r^{k+1} \right] \mid r^k  \right] = 0
	$.
\end{lemma}

The Q-function update can be performed online based on Least-squares (LS) methods using the data tuple $\left[ X^T_t, u_t \right]$, $\left[ X^T_{t+1}, u_{t+1} \right]$ and instantaneous cost $X^T_t S X_t+ c_2 u^2_t$ as shown in \cite{kiumarsi2014reinforcement}. Since update of Q-function involves update of symmetric $H^k$ matrix with dimension $3 \times 3$ and the scalar $r^k$ there are a total of $(3 \times 2) + 1 = 7$ independent elements so at least $7$ data tuples are required before an update can be made.

\subsection{Two timescale Algorithm} \label{subsec:TTSRL}
In this section we introduce the two timescale algorithm \cite{borkar1997stochastic}, \cite{leslie2004reinforcement} which is shown to iteratively recover the equilibrium control for the generic agent. The two timescale algorithm has a faster and a slower timescale. These updates happen at the concurrently but their \textit{speeds} are managed so that one appears to be faster than the other. The learning rates $\alpha_k$ and $\beta_k$ dictate the speed at which each update is made. They are chosen according to standard conditions for the two timescale algorithm \cite{borkar1997stochastic}. 
\begin{align}
\sum_{k=0}^{\infty} \alpha_k = \infty, \sum_{k=0}^{\infty} \beta_k = \infty, \sum_{k=0}^{\infty} (\alpha^2_k + \beta^2_k) < \infty
\\
\lim_{k \rightarrow \infty} \alpha_k = 0, \lim_{k \rightarrow \infty} \beta_k = 0, \lim_{k \rightarrow \infty} \alpha_k/\beta_k = 0
\end{align}

The two timescale algorithm updates the mean-field $\bar{z}^k$ at the slower timescale and the feedback control gain $L^k$ at the faster timescale. First the slower timescale update of $z^k$ is explained. 

The initial mean-field $\bar{z}^0$ is a $0$-latent LTI mean-field and it is updated at each iteration $k$, using an estimate of the $\mathcal{T}^L$ operator, so as to be a $k$-latent LTI mean-field. This operator is called the \textit{state aggregator} and is denoted by $\tilde{\mathcal{T}}^L$. It is an \textit{unbiased} estimate of $\mathcal{T}^L$ and it takes the average of the states of a finite set of agents in such a way to retain the unbiased nature of the aggregator. This is similar to the method used in \cite{subramanian2019reinforcement}.
\begin{equation} \label{eq:tts_mf_update}
\left[ \begin{array}{c} f^{k+1} \\ \bar{z}^{k+1}_{\tau+1} \end{array} \right] = \left[ \begin{array}{c}f^k \\ \bar{z}^k_{\tau} \end{array}\right] + \alpha_k \left(\tilde{\mathcal{T}}^L \left(\left[ \begin{array}{c}f^k \\ \bar{z}^k_{\tau} \end{array}\right], L^k \right) - \left[ \begin{array}{c}f^k \\ \bar{z}^k_{\tau} \end{array}\right] \right)
\end{equation}
This is the convex combination of the previous mean-field $\bar{z}^k$ and the intermediate mean-field $\tilde{\mathcal{T}}^L(\cdot, L^k)$.

Now we detail the faster timescale update of $L^k$. But first an issue needs to be addressed. From Section \ref{subsec:QlearningLQR} recall that Q-learning iteratively recovers the cost-minimizing control \textit{for time $t \geq \tau$}, for a $\tau$-latent mean-field . So to be able to use this technique in the two timescale algorithm, we need to ensure that at each iteration, $t \geq \tau$ where $\tau$ is the latency variable of $\bar{z}^k$. This means that although the mean-field is being updated at each $k$, the algorithm should be ensured to be in the linear region of the $\tau$-latent mean-field $\bar{z}^k$. 

Since at each $k$ the mean-field is a $k$-latent LTI mean-field, this requirement translates to $t \geq k$. At the start of the algorithm $t=0$ and $k=0$ (since $\bar{z}^0$ is an $0$-latent LTI mean-field) so the condition is trivially satisfied. Each iteration $k$ involves an update of the Q-function which takes at least 7 time steps (Section \ref{subsec:QlearningLQR}). This ensures $t \geq k$ for all time. This means the Q-learning method introduced in Section \ref{subsec:QlearningLQR} can be used to iteratively obtain the cost-minimizing control for the $\bar{z}^k$ for time $t \geq k$.

%Note that as $\bar{z}^{k}$ is a $k$-latent LTI mean-field, $\bar{z}^{k+1}$ will be a $(\tau + 1)$-latent LTI mean-field (Lemma \ref{lem:LTI2LTI}). As mean-field updates at a slower timescale, if current time $t \geq \tau$ then $t+1 \geq \tau + 1$ and so the future trajectory of the updated mean-field (trajectory after $t$) will always have linear dynamics. Hence, the Q-learning algorithm developed in Section \ref{subsec:QlearningLQR} can be used to update the feedback gains $L^k$ to optimally track the updated mean-field. This operates at the faster timescale in the two timescale algorithm.

The initial Q-function $Q^0$ is defined by positive semidefinite matrix $H^0$ and scalar $r^0$. The initial feedback gains $L^0$ can be computed using $H^0$ as shown in equation \eqref{eq:L_t}. Q-function at iteration $k$ has a structure quadratic in state and action as in equation \eqref{eq:Q_func},
\begin{equation} \label{eq:Q_func_inter}
Q^{k}(X_t, u_t) = \left[ \begin{array}{c} X_t \\ u_t \end{array} \right]^T H^{k} \left[ \begin{array}{c} X_t \\ u_t \end{array} \right] + r^{k}
\end{equation}
The intermediate Q-function $\tilde{Q}^k$ can be obtained as in equation \eqref{eq:Qupdate},
\begin{multline} \label{eq:Qinterupdate}
\tilde{Q}^{k}(X_t, u_t) = \left[ \begin{array}{c} X_t \\ u_t \end{array} \right]^T \left[ \begin{array}{cc} S & 0 \\ 0 & c_2 \end{array} \right] \left[ \begin{array}{c} X_t \\ u_t \end{array} \right] + \\
\gamma \min_{u_{t+1}} Q^{k}(X_{t+1}, u_{t+1})
\end{multline}
The intermediate Q-function $\tilde{Q}^k$ is defined by the matrix $\tilde{H}^k$ and scalar $\tilde{r}^k$,
\begin{equation} \label{}
\tilde{Q}^{k}(X_t, u_t) = \left[ \begin{array}{c} X_t \\ u_t \end{array} \right]^T \tilde{H}^{k} \left[ \begin{array}{c} X_t \\ u_t \end{array} \right] + \tilde{r}^{k}
\end{equation}
The intermediate feedback gain $\mathcal{G}(\bar{z}^{k},L^k)$ is generated as given in equation \eqref{eq:L_t}. 
\begin{equation}
\mathcal{G}(\bar{z}^{k},L^k) = - \left( \tilde{H}^{uu,k} \right)^{-1} \tilde{H}^{ux,k}
\end{equation}
The the updated feedback gains $L^{k+1}$ are obtained in standard stochastic optimization fashion, by taking a convex combination of the intermediate gain $\mathcal{G}(\bar{z}^{k},L^k)$ and previous gain $L^k$,
\begin{equation} \label{eq:tts_gain_update}
L^{k+1} = L^k + \beta_k \left( \mathcal{G}(\bar{z}^{k},L^k) - L^k \right)
\end{equation}
$Q^{k+1}$ is defined as,
\begin{equation*}
Q^{k+1} = Q^k + \beta_k (\tilde{Q}^k - Q^k)
\end{equation*} 
Algorithm \ref{alg:RL-LQMFG} presents the two timescale algorithm to recover the equilibrium control. 

\begin{algorithm} \label{alg:alg_TTSA}
	\caption{Learning algorithm for LQ-MFGs}
	\begin{algorithmic}[1]
		\STATE Initialize $\bar{z}^0$ a $0$-latent LTI mean-field s.t. $\bar{z}^0_0 = \mu_0$
		\STATE Initialize $H^0 > 0, r^0$.
		\STATE $t = 0$
%		\STATE Initialize $Q$ function.
		\FOR {$k = 0,1,2,...$}
%		\STATE Generate $L^k$ using $Q$ function
		\FOR {$i = 1,2,..,7$}
		\STATE Take action using $u^k_t = L^k X_t = L^k \left[ \begin{array}{c}
		z_t \\ \bar{z}^{k}_t
		\end{array} \right]$
		\STATE $t = t + 1$
		\ENDFOR
		\STATE Update mean-field $\bar{z}^k$, 
		\begin{multline*}
		\left[ \begin{array}{c} f^{k+1} \\ \bar{z}^{k+1}_{\tau+1} \end{array} \right] = \left[ \begin{array}{c}f^k \\ \bar{z}^k_{\tau} \end{array}\right] + \alpha_k \left(\tilde{\mathcal{T}}^L \left(\left[ \begin{array}{c}f^k \\ \bar{z}^k_{\tau} \end{array}\right], L^k \right) \right.\\
		\left. - \left[ \begin{array}{c}f^k \\ \bar{z}^k_{\tau} \end{array}\right] \right)
		\end{multline*}
%		\STATE $\mathcal{g}(\bar{z}^{k}) = K_N$
		\STATE Update Control gain $L^k$
		\begin{equation*}
		L^{k+1} = L^k + \beta_k \left( \mathcal{G}(\bar{z}^{k},L^k) - L^k \right)
		\end{equation*}
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

Now we show that the algorithm approaches the equilibrium control. First the algorithm is shown to recover the equilibrium mean-field in the following theorem. The proof is provided in the appendix.

\begin{theorem}
Under Assumption \ref{asm:boundforcontract}, as $k \rightarrow \infty$, the $(f^k, \bar{z}^k_{\tau})$-mean-field approaches the equilibrium mean-field.
\end{theorem}

The next lemma shows that the control $u^k_t = L^k X_t$ approaches the cost-minimizing control for the equilibrium mean-field for the future.

\begin{lemma}
Under Assumption \ref{asm:boundforcontract}, as $k \rightarrow \infty$, the control $u^k_t = L^k X_t$ approaches the cost-minimizing control for the $(f^k, \bar{z}^k_{\tau})$-mean-field, in the future.
\end{lemma}

Now we present the main result guaranteeing that the two timescale Q-learning based Algorithm \ref{alg:RL-LQMFG} will iteratively recover the equilibrium control.

\begin{theorem}\label{thm:TTSA}
Under Assumption \ref{asm:boundforcontract}, as $k \rightarrow \infty$, the control $u_t = L^k X_t$ approaches the cost-minimizing control for the equilibrium mean-field for $t \geq k$.
\end{theorem}

%\begin{theorem}\label{thm:TTSA}
%Under Assumption \ref{asm:boundforcontract}, Algorithm \ref{alg:RL-LQMFG} obtains the MFE $(\bar{z}^*, L^*)$ in the limit.
%\end{theorem}

The proof of this theorem uses convergence properties of the Q-update (Lemmas \ref{lem:H^k->H} and \ref{lem:r^k->r}), the contractive property of the operator $\mathcal{T}$ (Lemma \ref{lem:contract}) and the existence and uniqueness of the MFE (Theorem \ref{thm:exist_uniq_mfe}). The next section presents simulations to corroborate these results.

%\begin{algorithm}
%	\caption{Q-learning algorithm} \label{alg:RL-LQMFG}
%	\begin{algorithmic}[1]
%		\STaTE $\bar{z}^0 = \left( \bar{z}^0_t \right)_{t \in \mathbb{N}}$, $\bar{z}^0_0 = \mu_0$.
%		\STaTE $t = 0$
%		\FOR {$k = 0,1,2,...$}
%		\STaTE Initialize $Q$ function.
%		\FOR {$i = 1$ to $N$}
%		\STaTE Generate feedback gains $\hat{K}_i$ using $Q$ function
%		\STaTE $K_i = (1-\alpha_k)K_{i-1} + \alpha_k \hat{K}_i$
%		\FOR {$j = 1$ to $M$}
%		\STaTE Take action using $u_t = K_i \left[ \begin{array}{c}
%		z_t \\ \bar{z}^{k}_t
%		\end{array} \right]$
%		\STaTE update $Q$ function using reward at time $t$
%		\STaTE $t = t + 1$
%		\ENDFOR
%		%\STaTE Improve policy based on $Q$ function
%		\ENDFOR
%		\STaTE Generate $\hat{z}^{k+1}$ using feedback policy and state aggregator $\mathcal{T}^L$.
%		\STaTE $\bar{z}^{k+1} = (1-\beta_k)\bar{z}^{k} + \beta_k \hat{z}^{k+1}$
%		\ENDFOR
%	\end{algorithmic}
%\end{algorithm}


%\begin{proof}
%Given the mean-field $z^*_t$, computing the optimal control is the solution to a Gaussian Linear-Quadratic Tracking (LQT) problem. We follow methods similar to \cite{chen2012identification} and \cite{wang2014discrete} to obtain the solution. We start by expressing 
%\begin{align*}
%J^{k}(u_t,z_\tau) & = \sum^{n-1}_{t=0} \beta^t \EE\left[ (z_t - z_\tau)^2 +ru_t^2 \right] \\ 
%& = \sum^{n-1}_{t=0} \beta^t \EE\left[ z_t^2 -2z_\tau z_t + z_t^{*2} +ru_t^2 \right]
%\end{align*}
%in a complete square form. First we introduce two telescoping sums.
%\begin{align*}
%& \beta^n S z^2_n - S z^2_0 = \sum^{n-1}_{t=0} \beta^t \left(\beta S z_{t+1}^2 - S z^2_t \right) \\
%= & \sum^{n-1}_{t=0} \beta^t \left(\beta S \left(az_t+bu_t+\sigma w_t \right)^2 - S z^2_t \right) \\
%= & \sum^{n-1}_{t=0} \beta^t \left(\beta S \left(az_t+bu_t+\sigma w_t \right)^2 \right.\\
%& - \left. \left(a^2\beta S + 1 -\frac{(abS \beta)^2}{r + b^2 S \beta} \right) z^2_t \right) \hspace{0.1cm} \text{(using \eqref{eq:S})} \\
%= & \sum^{n-1}_{t=0} \beta^t \left(2a \beta S \left(bu_t+\sigma w_t \right)z_t + \beta S \left(bu_t+\sigma w_t \right)^2 \right.\\
%& - \left. \left( 1 -\frac{(abS \beta)^2}{r + b^2 S \beta} \right) z^2_t \right)
%\end{align*}
%\begin{align*}
%\hspace{-0.5cm} \sum^{n-1}_{t=0} \beta^t z^2_t =  & S z^2_0 - \beta^n S z^2_n  + \sum^{n-1}_{t=0} \beta^t \left(2a \beta S \left(bu_t+\sigma w_t \right)z_t \right.\\
%& \left. + \beta S \left(bu_t+\sigma w_t \right)^2 - \frac{(abS \beta)^2}{r + b^2 S \beta} z^2_t \right)
%\end{align*}
%and another telescoping sum,
%\begin{align*}
%& \beta^n \lambda_n z_n - \lambda_0 z_0 = \sum^{n-1}_{t=0} \beta^t \left( \beta \lambda_{t+1} z_{t+1} - \lambda_t z_t\right) \\
%& = \sum^{n-1}_{t=0} \beta^t \left( \beta \lambda_{t+1} \left(az_t+bu_t+\sigma w_t \right) - \lambda_t z_t\right)
%\end{align*}
%using \eqref{eq:lambda_t} we can also say,
%\begin{equation*}
%\lambda_t z_t = \left( a \beta - \frac{ab^2 S \beta^2}{r + b^2 S \beta} \right)\lambda_{t+1}z_t - z^*_t z_t
%\end{equation*}
%substituting these sums into $J^{k}$ we get,
%\begin{align*}
%& J^{k}(u_t,z_\tau) = \sum^{n-1}_{t=0} \beta^t \EE\left[ z_t^2 -2z_\tau z_t + z_t^{*2} +ru_t^2 \right] \\
%& = \EE \left[ S z^2_0 - \beta^n S z^2_n + \sum^{n-1}_{t=0} \beta^t \left[ \frac{(abS)^2}{r + b^2 S} z^2_t \right. \right.\\
%& \left. \left. + 2a S \beta\left(b u_t + \sigma w_t \right) z_t + S \beta \left( bu_t + \sigma w_t \right)^2 \right]  \right.\\
%& + 2\lambda_0 z_0 - 2 \beta^n \lambda_n z_n + \sum^{n-1}_{t=0}\beta^t \left[ 2\beta \lambda_{t+1} \left( az_t + bu_t  \right. \right. \\
%& \left. + \sigma u_t \right) \left. \left. -2 \lambda_t z_t - 2z^*_t z_t + z^{*2}_t + r u^2_t \right] \right]
%\end{align*}
%\begin{align*}
%& = \EE \left[ S z^2_0 - \beta^n S z^2_n + 2\lambda_0 z_0 - 2 \beta^n \lambda_n z_n \right.\\
%&  + \sum^{n-1}_{t=0} \beta^t \left[ \frac{(abS)^2}{r + b^2 S} z^2_t + 2a S \beta\left(b u_t + \sigma w_t \right) z_t \right. \\
%& + \left. S \beta \left( bu_t + \sigma w_t \right)^2 \right] + \sum^{n-1}_{t=0}\beta^t \left[ 2\beta \lambda_{t+1} \left(bu_t + \sigma u_t \right) \right. \\
%& \left. \left. + \frac{2ab^2S}{r + b^2 S \beta}\lambda_{t+1}z_t + z^{*2}_t + r u^2_t \right] \right]
%\end{align*}
%\begin{align*}
%& = \EE \left[ S z^2_0 - \beta^n S z^2_n + 2\lambda_0 z_0 - 2 \beta^n \lambda_n z_n + \sum^{n-1}_{t=0} \beta^t \left[ S \beta w^2_t \right] \right.\\
%& + \sum^{n-1}_{t=0} \beta_t \left[ z^{*2}_t - \frac{(b \beta)^2}{r + b^2 S \beta}\lambda^2_{t+1} \right] \\
%& + 2 \sum^{n-1}_{t=0}\beta^t \sigma \beta \left( S(az_t + bu_t) + \lambda_{t+1}\right)w_t \\
%& + \sum^{n-1}_{t=0} (r + b^2 S \beta)u^2_t + 2a S \beta b u_t z_t + 2 \beta b \lambda_{t+1} u_t \\
%& \left. + \frac{2 a b^2 S \beta^2}{r + b^2 S \beta} \lambda_{t+1} z_t + \frac{(a b S \beta)^2}{r + b^2 S \beta}z^2_t + \frac{(b \beta)^2}{r + b^2 S \beta}\lambda^2_{t+1} \right]
%\end{align*}
%\begin{align*}
%& = \EE \left[ S z^2_0 - \beta^n S z^2_n + 2\lambda_0 z_0 - 2 \beta^n \lambda_n z_n + \sum^{n-1}_{t=0} \beta^t \left[ S \beta w^2_t \right]  \right.\\
%& + \sum^{n-1}_{t=0} \beta_t \left[ z^{*2}_t - \frac{(b \beta)^2}{r + b^2 S \beta}\lambda^2_{t+1} \right] \\
%& + 2 \sum^{n-1}_{t=0}\beta^t \sigma \beta \left( S(az_t + bu_t) + \lambda_{t+1}\right)w_t \\
%& + \left. \sum^{n-1}_{t=0} (r + b^2 S \beta) \left( u_t + \frac{(b \beta)^2}{r + b^2 S \beta} \left( a S z_t + \lambda_{t+1} \right) \right)^2 \right]
%\end{align*}
%\begin{align*}
%& =  S z^2_0 + 2\lambda_0 z_0 - \beta^n \EE \left[S z^2_n - 2\lambda_n z_n \right] + S \sum^{n}_{t=1} \beta^t \\
%& + \sum^{n-1}_{t=0} \beta_t \left[ z^{*2}_t - \frac{(b \beta)^2}{r + b^2 S \beta}\lambda^2_{t+1} \right] \\
%& + \EE \left[ \sum^{n-1}_{t=0} (r + b^2 S \beta) \left( u_t + \frac{(b \beta)^2}{r + b^2 S \beta} \left( a S z_t + \lambda_{t+1} \right) \right)^2 \right]
%\end{align*}
%
%This proves that the optimal control is given by \eqref{eq:u_t}-\eqref{eq:lambda_t}.
%\end{proof}

%\begin{assumption} \label{asm:k_2}
%$|k_2| = \left|  \frac{r a \beta}{r + b^2 S \beta} \right| < 1$
%\end{assumption}
%
%\begin{lemma} \label{lem:lambda_bdd}
%If assumption \ref{asm:k_2} is satisfied then the $\lambda_t$ is bounded and hence $u^*_t$ is also bounded.
%\end{lemma}

%\section{Policy Iteration}
%
%This is the mean-field dynamics update operator $\mathcal{T}$,
%\begin{equation*}
%\bar{z}^{k+1} = \mathcal{T}_1(\bar{z}^{k}, u^k(\bar{z}^{k})) = \mathcal{T} (\bar{z}^{k})
%\end{equation*}
%From the definition of the MFE \eqref{def:mfe} $z^* = \mathcal{T}_1(z^*,u(z^*))$ and $u^*$ is the control that minimizes $J(z^*,u)$. Hence if we prove that $\mathcal{T}$ is a contraction mapping then it will eventually converge to the MFE.
%\begin{theorem}
%The operator $\mathcal{T}$ is a contraction mapping on the $\ell^{\infty}$ space if,
%\begin{equation} \label{asm:contract}
%\left| a + a b S k_1 \right| + \left| b \frac{k_1}{1 - k_2}  \right| < 1 \,.
%\end{equation}
%and assumption \eqref{asm:k_2} is satisfied. Moreover if a sequence $\bar{z} \in \ell^{\infty}$ then, $\mathcal{T}(\bar{z}) \in \ell^{\infty}$.
%\end{theorem}
%\begin{proof}
%We start by introducing two sequences $\bar{z}^{k}, \hat{z}^k \in \ell^{\infty}$. $\tilde{z}^k$ is the difference between the two sequences $\tilde{z}^k = \bar{z}^{k}-\hat{z}^k$. $\bar{z}^{k+1}, \hat{z}^{k+1}$ are the transformed versions of these sequences $\bar{z}^{k+1} = \mathcal{T}(\bar{z}^{k})$ and $\hat{z}^{k+1} = \mathcal{T}(\hat{z}^k)$. and $\tilde{z}^{k+1}$ is the difference between these two sequences $\tilde{z}^{k+1} = \bar{z}^{k+1}-\hat{z}^{k+1}$. using equation \eqref{eq:T},
%\begin{equation*}
%\bar{z}^{k+1}_{t+1} = \left(a + a b S k_1  \right) \bar{z}^{k}_t - b \frac{k_1}{k_2}\sum_{i=t+1}^{\infty} k_2^{i-t} \bar{z}^{k}_i \,,
%\end{equation*}
%and
%\begin{equation*}
%\hat{z}^{k+1}_{t+1} = \left(a + a b S k_1  \right) \hat{z}^k_t - b \frac{k_1}{k_2}\sum_{i=t+1}^{\infty} k_2^{i-t} \hat{z}^k_i \,,
%\end{equation*}
%$\forall t \in \mathbb{N}$ and $\bar{z}^{k+1}_0 = \hat{z}^{k+1}_0 = \EE z_0$, Taking the difference we get,
%\begin{equation*}
%\tilde{z}^{k+1}_{t+1} = \left(a + a b S k_1  \right) \tilde{z}^k_t - b \frac{k_1}{k_2}\sum_{i=t+1}^{\infty} k_2^{i-t} \tilde{z}^k_i \,,
%\end{equation*}
%\begin{align*}
%\left| \tilde{z}^{k+1}_{t+1} \right| & \leq \left| \left(a + a b S k_1  \right) \tilde{z}^k_t \right| + \left| b \frac{k_1}{k_2}\sum_{i=t+1}^{\infty} k_2^{i-t} \tilde{z}^k_i \right| \,, \\
%& \leq \left| a + a b S k_1 \right| \left\lvert{\tilde{z}^k} \right\lvert_{\infty} + \left| b \frac{k_1}{k_2}  \right| \sum_{i=t+1}^{\infty} |k_2^{i-t}| \left\lvert \tilde{z}^k \right\lvert_{\infty} \,, \\
%& \leq \left| a + a b S k_1 \right| \left\lvert{\tilde{z}^k} \right\lvert_{\infty} + \left| b \frac{k_1}{1 - k_2}  \right| \left\lvert \tilde{z}^k \right\lvert_{\infty} \,, \\
%& \leq \left( \left| a + a b S k_1 \right| + \left| b \frac{k_1}{1 - k_2}  \right| \right) \left\lvert \tilde{z}^k \right\lvert_{\infty} \hspace{0.2cm} \forall t \in \mathbb{N}
%\end{align*}
%Hence by using the assumption \eqref{asm:contract} we obtain the contraction. Its easy to see that for a bounded $\bar{z}$, $\mathcal{T}(\bar{z})$ is also bounded by repeating the above given process with $\hat{z}^k$ as a sequence of all $0$s.
%\end{proof}

%\section{Policy Iteration algorithm and analysis}
%
%as the optimal control \eqref{eq:u_t}-\eqref{eq:lambda_t} have a non-causal structure, there is an infinite sum that needs to be computed in order to obtain the mean-field at the next time step $\bar{z}^{k+1}$. So in this section we propose an implementable algorithm to iterative approximate the MFE. We also show that this algorithm can approximate the MFE up to a certain error tolerance. We also achieve bounds on optimality of the proposed algorithm.
%\begin{algorithm}
%	\caption{Policy Iteration algorithm} \label{alg:policyiter}
%	\begin{algorithmic}[1]
%		\STaTE $\bar{z}^0 = \left( \bar{z}^0_t \right)_{t \in \mathbb{N}} \in \ell^{\infty}$, $\bar{z}^0_0 = \EE [\mu_0]$.
%		\FOR {$k = 0,1,2,...$}
%		\STaTE Calculate $u^k_t$ using, $$ u^k_t = k_1 (aSz_t^k + \lambda^k_{t+1}) $$ where $S$ is the positive solution to the aRE \eqref{eq:S} and $$ \lambda^k_t  = -\sum_{i=t}^{t+N} k_2^{i-t} \bar{z}^{k}_i \,, $$
%		\STaTE Calculate $\bar{z}^{k}$ using, $$ \bar{z}^{k+1} = \mathcal{T}_1(\bar{z}^{k}, u^k(\bar{z}^{k})) = \mathcal{T} (\bar{z}^{k}) $$
%		\ENDFOR
%	\end{algorithmic}
%\end{algorithm}

%\subsection{Error bounds on generated mean-fields}
%\subsection{Optimality bounds}
%
%
